Towards Reliable Uncertainty Quantification via Deep Ensembles in Multi-output Regression Task

This study aims to comprehensively investigate the deep ensemble approach, an approximate Bayesian inference, in the multi-output regression task for predicting the aerodynamic performance of a missile configuration. To this end, the effect of the number of neural networks used in the ensemble, which has been blindly adopted in previous studies, is scrutinized. As a result, an obvious trend towards underestimation of uncertainty as it increases is observed for the first time, and in this context, we propose the deep ensemble framework that applies the post-hoc calibration method to improve its uncertainty quantification performance. It is compared with Gaussian process regression and is shown to have superior performance in terms of regression accuracy ($\uparrow55\sim56\%$), reliability of estimated uncertainty ($\uparrow38\sim77\%$), and training efficiency ($\uparrow78\%$). Finally, the potential impact of the suggested framework on the Bayesian optimization is briefly examined, indicating that deep ensemble without calibration may lead to unintended exploratory behavior. This UQ framework can be seamlessly applied and extended to any regression task, as no special assumptions have been made for the specific problem used in this study.

==> update.tex <==
221206
- Intro의 EGO 문단을 UQ in engineering의 활용 방안정도만 강조하는 식으로 간략하게 정리
- 그리고 UQ의 필요성을 EGO 뿐만 아니라 interpretability in decision making - e.g., risk assessment로 해석하기. 예를 들어 CFD 에서 데이터가 나오고 이를 바탕으로 regression했다고 하자. --> 이 때 이러한 regression을 바탕으로 한 예측에서는 불확실성이 데이터로부터 나오는 uncertainty, 근사모델에서 나오는 uncertainty가 있는데 이를 구분하고 각각이 얼만큼인지 알아야 이후 reasonable, realistic한 의사 결정 가능
- GPR의 내용도 v1에 비해 줄임. 세부적인 원리 지움.
- BNN은 내용을 더줄여야 됨. 그냥 BNN이 ~한 한계를 가져서 approximate Bayesian이 필요하다 이정도만 얘기해주면되지 v1처럼 BNN에 대해 많이 언급할 필요가 없음.
